Learning to cluster in order to transfer across domains and tasks

This paper introduces a novel method to perform transfer learning across domains and tasks, formulating it as a problem of learning to cluster. The key insight is that, in addition to features, we can transfer similarity information and this is sufficient to learn a similarity function and clustering network to perform both domain adaptation and cross-task transfer learning. We begin by reducing categorical information to pairwise constraints, which only considers whether two instances belong to the same class or not. This similarity is category-agnostic and can be learned from data in the source domain using a similarity network. We then present two novel approaches for performing transfer learning using this similarity function. First, for unsupervised domain adaptation, we design a new loss function to regularize classification with a constrained clustering loss, hence learning a clustering network with the transferred similarity metric generating the training inputs. Second, for cross-task learning (i.e., unsupervised clustering with unseen categories), we propose a framework to reconstruct and estimate the number of semantic clusters, again using the clustering network. Since the similarity network is noisy, the key is to use a robust clustering algorithm, and we show that our formulation is more robust than the alternative constrained and unconstrained clustering approaches. Using this method, we first show state of the art results for the challenging cross-task problem, applied on Omniglot and ImageNet. Our results show that we can reconstruct semantic clusters with high accuracy. We then evaluate the performance of cross-domain transfer using images from the Office-31 and SVHN-MNIST tasks and present top accuracy on both datasets. Our approach doesn't explicitly deal with domain discrepancy. If we combine with a domain adaptation loss, it shows further improvement.

==> sections/experiments.tex <==
\section{Experiments}
We evaluate the effectiveness of transferring pairwise semantic similarity in two scenarios. For the unsupervised cross-task transfer learning described in section \ref{crosstask}, we applied the learned constraints on an unlabeled image dataset with unseen categories to do constrained clustering. We then evaluate its clustering performance to see if semantically coherent clusters are reconstructed. For the unsupervised cross-domain transfer learning in section \ref{crossdomain}, we evaluate the performance with an image classification task.

\subsection{Unsupervised Cross-Task Transfer Learning} \label{crosstaskexp}

\subsubsection{Setup} \label{crosstaskSetup}
The \textbf{Omniglot} dataset \citep{Lake1332} contains 1623 different handwritten characters and each of them has 20 images drawn by different people. The characters are from 50 different alphabets and were separated to 30 background sets $Omniglot_{bg}$ and 20 evaluation sets $Omniglot_{eval}$ by the author. We use the $Omniglot_{bg}$ as the auxiliary dataset and the $Omniglot_{eval}$ as the target data. The total number of characters in $Omniglot_{bg}$ is 964, which can be regarded as the number of categories available to learn the semantic similarity. 

\textbf{The $S$ function} has a backbone neural network with four 3x3 convolution layers followed by 2x2 max-pooling with stride 2. The architecture is illustrated in figure [X]. All hidden layers are followed by batch normalization [REF] and rectified linear unit. To prepare the inputs for training, the images from $Omniglot_{bg}$ were resized to 32x32 and normalized to zero mean with unit standard deviation. Each mini-batch has size of 100 and is sampled from random 20 characters to make sure the amount of similar pairs is reasonable. After pair enumeration, there are 10000 pairs subject to the loss function, which is a two-class cross entropy loss. The ground-truth similarity is obtained by converting the categorical labels. $S$ is optimized by stochastic gradient decent and is the only part trained in a supervised manner in this section.

\textbf{The Constrained Clustering Networks (CCN)} is used to reconstruct the semantic clusters in the target dataset. We called the neural network as CCN if it only use the CCL for the loss. The network has four 3x3 convolution layers followed by 2x2 max-pooling with stride 2, one hidden fully-connected layer, and one cluster assignment layer which is also fully connected. The number of output nodes in the last layer is equal to the number of potential cluster in target data. The output distribution is enumerated in pairs before sending to CCL. The network is trained end-to-end and optimized by stochastic gradient decent with randomly sampled 100 images per mini-batch. Note the $S$ function used by $L_{clust}$ is fixed during the optimization. The input data preparation is the same as above, except now the data is from $Omniglot_{eval}$. Specifically, during the training, the same mini-batch is given to both $S$ and CCN. The dense pairwise similarity predictions from $S$ are sent to $L_{clust}$ and are then fully utilized. The only hyper-parameter in $L_{clust}$ is the  $\sigma$, and we set it to 2 for all our experiments. 

$Omniglot_{eval}$ contains 20 alphabets and each one can be used as a standalone dataset. The 20 target datasets contain a varied number (20 to 47) of characters. Therefore we can evaluate the reconstruction performance under a varied number of ground-truth clusters. We tested the situations when the number of character ($K$) in an alphabet is known and unknown. When $K$ is known, we set the target number of clusters in the clustering algorithm equal to true number of characters. If $K$ is unknown, the common practice is to set it to a large number so that the data from different categories will not be forced to be in the same cluster. In the experiment, we simply set $K$ to 100, which is much larger than the largest dataset (47).

All constrained clustering algorithms can be used to reconstruct the semantic clusters for our problem. Since there are mis-predictions in $S$, robustness to noise is the most important factor. Here we include all four types of constrained clustering introduced in section (REF) as the baselines. We provide the full set of pairwise constraints to all algorithms including ours. In other words, given an alphabet of 20 characters, it will contains 400 images and 16000 predicted similarities from $S$ (note the $S$ makes predictions in both orders of a pair and for self pairs). The full pairwise similarities were presented to all algorithms in random order, while we empirically found it has no noticeable effect on results. We pick the baseline approaches based on code availability and scalability with respect to the number of pairwise constraints. Therefore we have shown results for kmeans, NMF\_LP [REF], LCS [REF], ITML [REF], SKKm [REF], SKLR [REF], SKMS [REF], CSP [REF], and MPCKMeans [REF] as our baselines. We use the default parameters for each algorithm \ZK{Are these not tunable?} provided by original author except for $K$, the number of cluster. We use the same normalized images used in CCN for all algorithms.

The evaluation uses two clustering metrics. The first is normalized-mutual information (NMI) \citep{strehl2002cluster} which is widely used for clustering. The second one is the clustering accuracy (ACC) \citep{yang2010image}. The ACC metric first finds the one-to-one matching between predicted clusters and ground-truth labels, and then calculates the classification accuracy based on the mapping. All data outside the matched clusters will be regarded as mis-predictions. To get high ACC, the algorithm has to generate coherent clusters where each cluster includes most of the data in a category; otherwise the score drops quickly. Therefore ACC provides better discrimination to evaluate whether the semantic clusters have been reconstructed well.

\begin{table}[]
\centering
\caption{Transferring semantic similarity from $Omniglot_{bg}$ to $Omniglot_{eval}$. The ACC and NMI without brackets sets the number of clusters equal to the ground-truth. The performance is averaged across 20 alphabets which have 20 to 46 letters. The 100 in brackets means the algorithms used $K=100$ to mimic the situation where the actual number of semantic categories is unknown. The characteristics of how each algorithm utilizes the pairwise constraints are marked in the "Constraints used in" column, where metric stands for the metric learning of feature representation. }
\label{crosstask-omnilgot}
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{Constraints used in} & \multirow{2}{*}{ACC} & \multirow{2}{*}{ACC (100)} & \multirow{2}{*}{NMI} & \multirow{2}{*}{NMI (100)} \\
                & Metric & Clustering &            &                              &                             &                              \\ \midrule
kmeans          &     &      & 21.7\%    & 18.9\%  & 0.353   & 0.464  \\ 
NMF\_LP         &     &      & 22.2\%    & 16.3\%  & 0.372   & 0.498  \\
LCS             &     &      & 23.6\%    & 18.0\%  & 0.376   & 0.500  \\
ITML            & o   &      & 56.7\%    & 47.2\%  & 0.674   & 0.727  \\
SKMS            & o   &      & -         & 45.5\%  & -       & 0.693  \\
SKKm            & o   &      & 62.4\%    & 46.9\%  & 0.770   & 0.781  \\
SKLR            & o   &      & 66.9\%    & 46.8\%  & 0.791   & 0.760  \\
CSP             &     & o    & 62.5\%    & 65.4\%  & 0.812   & 0.812  \\
MPCKMeans       & o   & o    & 81.9\%    & 53.9\%  & 0.871   & 0.816  \\ \midrule
CCN (Ours)      & o   & o    & \textbf{82.4\%}    & \textbf{78.1\%}  & \textbf{0.889}   & \textbf{0.874}  \\ \bottomrule                     
\end{tabular}
\end{table}

\subsubsection{Results and Discussions} \label{crosstask_result}
The results are summarized in table \ref{crosstask-omnilgot}, which reports the average performance over the 20 alphabets. Our approach achieved the top performance on both metrics. The CCN demonstrates promising robustness on the challenging scenario of unknown $K$. It achieved 78.1\% average accuracy. Compared with 82.4\% when $K$ is known, CCN has a relatively small drop. If comparing it with the second best algorithm, CSP, which is 65.4\%, CCN outperform it with a large gap. The classical approach MPCKMeans works surprisingly well when the number of clusters is known, but its performance dropped dramatically from 81.9\% to 53.9\% when $K$ is set to a larger number. If we look the performance of 20 individual alphabets (see supplementary), CCN achieved 94\% clustering accuracy on \textit{Old Church Slavonic Cyrillic}, which has 45 characters. Therefore the results show the feasibility of reconstructing semantic clusters using only noisy similarity predictions.

\textbf{When to use the semantic similarity?} The experiments in table \ref{crosstask-omnilgot} show a clear trend that utilizing the pairwise constraints jointly for both metric learning and minimizing the clustering loss achieves the best performance, including both MPCKMeans and CCN. In the case of unknown number of clusters, where we set $K=100$, the algorithms that use constraints to optimize clustering loss have better robustness, for example, CSP and CCN. The third group (ITML, SKMS, SKKm, and SKLR) that only use constraints for metric learning significantly outperformed the group that does not use it (kmeans,NMF\_LP,LCS). However, their performance are still far behind CCN. Our results confirm the importance of jointly optimizing the metric and clustering.

\textbf{The robustness} of the algorithm against noisy similarity prediction is the key factor to enable the cross-task transfer framework. To our best knowledge, table \ref{crosstask-omnilgot} is the first comprehensive robustness comparisons using the predicted constraints learned from real data instead of converting from ground-truth labels. The accuracy of $S$ in our experiment were shown in appendix [REF] and demonstrated the reasonable performance of $S$ which is on par with MatchingNet [REF]. After binarizing the prediction at 0.5 probability, the similar pair recall, similar pair precision, dissimilar pair recall, and dissimilar pair precision are [X,X,X,X], accordingly. The binarized predictions are better than random guess, but are still far from high accuracy. Therefore it is very challenging for constrained clustering. The visualization of the robustness range of CCN are provided in the appendix [REF], and shows that the robustness is related to the large amount of pairs been involved in a mini-batch. We hypothesize that during the optimization, the gradients from wrongly predicted pairs are canceled out by each other or by the correctly predicted pairs. Therefore the overall gradient still moves the solution towards a better clustering result. Finding the reason of robustness is not the focus of this paper so we left it to future work.\ZK{There is a paper I saw that says DNNs are pretty robust to label noise}

\textbf{How to predict $K$?} Inferring the number of clusters ($NC$) is a hard problem, but with the pairwise similarity information it becomes feasible. For evaluation, we compute the difference between the number of dominant clusters ($NDC$) and the true number of categories ($NC^{gt}$) in a dataset. We use a naive definition for $NDC$, which is the number of clusters that have size larger than expected size when data is sampled uniformly. In other words, $NDC=\sum_{i=1}^{K}{[C_i>=E[C_i]]}$, where $[\cdot]$ is an Iverson Bracket and $C_i$ is the size of cluster $i$. For example, $E[C_i]$ will be 10 if the alphabet has 1000 images and $K=100$. Then the average difference ($ADif$) is calculated by $ADif=\frac{1}{|D|}\sum_{d\in{D}}{|NDC_d-NC_d^{gt}|}$, where $d$ (i.e., alphabet) is a dataset in $D$. A smaller $ADif$ indicates a better estimate of $K$. CCN achieves a score of 6.35 (see supplementary). We compare this with the baseline approach SKMS [REF], which doesn't require a given $K$ and supports a pipeline to estimate $K$ automatically (therefore we only put it in to the column $K=100$ in table \ref{crosstask-omnilgot}.). SKMS gets 16.3. Furthermore, 10 out of 20 datasets from CCN's prediction have a difference between $NDC_d$ and $NC_d^{gt}$ smaller or equal to 3, which shows the feasibility of estimating $K$ with predicted similarity.

\subsection{Unsupervised Cross-Domain Transfer Learning}
\subsubsection{Setup}
We now describe our experiments on the cross-domain unsupervised adaptation task. \textbf{Office-31} \citep{Saenko2010} has images from 31 categories of office objects. The 4652 images are obtained from three domains: Amazon, DSLR, and Webcam. The dataset is the standard benchmark for evaluating domain adaptation performance in computer vision. We experiment all six combinations: $A \rightarrow W$, $A \rightarrow D$, $D \rightarrow A$, $D \rightarrow W$, $W \rightarrow A$, $W \rightarrow D$, and report the average accuracy based on five random experiments for each setting.

\textbf{The $S$ function} uses the ImageNet pre-trained Resnet-18 as the backbone network. The architecture is illustrated in figure [REF]. The semantic similarity is trained with 1000 categories in ImageNet. The training process is the same as section \ref{crosstaskSetup} except the images are resized to 224.

We follow the standard protocols using deep neural networks \citep{LongZ0J17,ganin2016domain} for unsupervised domain adaptation. During the training, all source data and target data are used. Each mini-batch is constructed by 32 labeled samples from source and 96 unlabeled samples from target. Since the target dataset has no label and could only be randomly sampled, it is crucial to have sufficient mini-batch size to make similar pairs be sampled. The loss function used in our approach is equation \eqref{eq:Lda} and is optimized by stochastic gradient decent. The CCL and DANN with ResNet [REF] backbone are implemented with Torch.

The comparison is made with state-of-the-art approaches includes Deep Domain Confusion (DDC) \citep{tzeng2014deep}, Deep Adaptation Network (DAN) \citep{LongC0J15}, Domain-adversarial training of neural networks (DANN, also called RevGrad in some literatures) \citep{ganin2016domain}, and Joint Adaptation Networks (JAN) \citep{LongZ0J17}. To emphasize positive transfer, we added an extra column to compare the gain on top of source-only training, which directly apply the learned classifier from source to target and is the baseline of the comparison.

\begin{table}[]
	\centering
	\caption{The performance of unsupervised transfer across domains on Office-31 dataset. The base networks used in all approaches are pre-trained with auxiliary dataset (ImageNet). The "Gain" column shows the gained performance compared with the classifiers trained only with source data. The first five rows directly come from \cite{LongZ0J17}. The $S^{Oracle}$ in the last row always gives the right prediction.}.
	\label{tab:office31_results}
	\begin{tabular}{@{}lcccccccc@{}}
		\toprule
		& A $\rightarrow$ W & D $\rightarrow$ W & W $\rightarrow$ D & A $\rightarrow$ D & D $\rightarrow$ A & W $\rightarrow$ A & Avg & Gain        \\ \midrule
        Backbone:AlexNet & & & & & & & &  \\
		Source-Only      & 61.6 & 95.4 & 99.0 & 63.8 & 51.1 & 49.8 & 70.1 & - \\
		DDC              & 61.8 & 95.0 & 98.5 & 64.4 & 52.1 & 52.2 & 70.6 & +0.5 \\
		DAN              & 68.5 & 96.0 & 99.0 & 67.0 & 54.0 & 53.1 & 72.9 & +2.8 \\
        DANN (RevGrad)             & 73.0 & 96.4 & 99.2 & 72.3 & 53.4 & 51.2 & 74.3 & +4.2 \\
		JAN-A            & 75.2 & 96.6 & 99.6 & 72.8 & 57.5 & 56.3 & 76.3 & +6.2 \\ \midrule
		%Resnet-50 source & 68.4 & 96.7 & 99.3 & 68.9 & 62.5 & 60.7 & 76.1 & +6.0 \\ \midrule
		%VGG16 source     & 67.6 & 96.1 & 99.2 & 73.9 & 58.2 & 57.8 & 75.5 & - \\
		%CMD              & 77.0 & 96.3 & 99.2 & 79.6 & 63.8 & 63.3 & 79.9 & +4.4 \\ \midrule
		%Alexnet source   & 60.9 & 92.9 & 98.4 & 61.2 & 49.8 & 47.7 & 68.5 & - \\
		%Alexnet SCCN     & 64.1 & 95.1 & 99.0 & 64.6 & 52.4 & 52.0 & 71.2 & +2.7 \\ \midrule
        Backbone:Resnet-18 & & & & & & & &  \\
		Source-Only                & 66.8 & 92.8 & 96.8 & 67.1 & 51.4 & 53.0 & 71.3 & - \\
        DANN (RevGrad)             & 73.2 & 97.0 & \textbf{99.0} & 69.3 & 58.0 & 57.8 & 75.7 & +4.4 \\
        CCL (ours)             & 76.7 & 97.3 & 98.2 & 71.2 & 61.0 & 60.5 & 77.5 & +6.2 \\
        CCL+DANN        & \textbf{78.2} & \textbf{97.4} & 98.6 & \textbf{73.5} & \textbf{62.8} & \textbf{60.6} & \textbf{78.5} & \textbf{+7.2} \\ \bottomrule
        %CCL with $S^{Oracle}$      & 99.8 & 100.0 & 99.8 & 98.8 & 97.1 & 92.8 & 98.0 & \\ \bottomrule
        %Backbone:Resnet-34 & & & & & & & &  \\
        %Source-Only        & 73.1 & 96.4 & 98.8 & 73.8 & 63.2 & 62.1 & 77.9 & - \\
        %DANN (RevGrad)     & 78.1 & 97.4 & 99.3 & 75.8 & 63.6 & 61.9 & 79.3 & +1.4 \\
        %CCL (ours)          & 78.0 & 96.6 & 99.3 & 78.9 & 67.8 & 66.2 & 81.1 & +3.2 \\
        %CCL+DANN           & 80.9 & 97.2 & 99.4 & 81.6 & 67.2 & 65.9 & 82.0 & +4.1 \\ \bottomrule
        %Resnet-50 source           & 74.3 & 96.8 & 98.8 & 79.5 & 61.2 & 60.6 & 78.5 & - \\ 
	\end{tabular}
\end{table}

\subsubsection{Results and Discussions}
The results are summarized in table \ref{tab:office31_results}. Our approach (CCL) demonstrates a strong performance boost for the unsupervised cross-domain transfer problem. It reaches 77.5\% average accuracy which gained 6.2 points from the 71.3\% source-only baseline. Although our approach merely transfers more information from the auxiliary dataset, it shows a larger performance gain compared to the DANN (+4.4), which is a strong approach to explicitly minimize the domain discrepancy. When combining DANN with CCL, the performance is further boosted. This indicates that CCL helps mitigate the transfer problem in a certain way that is orthogonal to minimizing the domain discrepancy. We observe the same trend when using a deeper backbone network, i.e, ResNet-34. In such a  case the average accuracy achieved is 77.9\%, 81.1\% and 82\% for source-only, CCL and CCL+DANN, respectively, though we used exactly the same $S$ as before (with ResNet-18 backbone for $S$)\ZK{VERIFY!}. This indicates that the information carried in the similarity predictions is not equivalent to transferring feature with deeper networks.

Since our source-only baseline has similar performance to \cite{LongZ0J17}, we make a comparison to the state-of-the-art JAN in terms of gained points and see CCL has on-par result. It gives a clear idea that by transferring extra information, it helps mitigating the domain shifting problem as significant as learning feature representation that minimize domain discrepancy. Since previous research heavily focused on the latter part, we advocate combining different aspects to achieve the best performance for domain adaptation.

We also evaluated CCL on another widely compared scenario, which transfer from color Street View House Numbers images (SVHN) \citep{Netzer2011} to gray hand-written digits (MNIST) \citep{lecun1998mnist}. The results are presented in appendix [REF] and show CCL out perform state-of-the art by a large margin.


==> sections/introduction.tex <==
\section{Introduction}

Supervised learning has made significant strides in the past decade, with substantial advancements arising from the use of deep neural networks. However, a large part of this success has come from the existence of extensive labeled datasets. In many situations, it is not practical to obtain such data due to the amount of effort required or when the task or data distributions change dynamically. To deal with these situations, the fields of transfer learning and domain adaptation have explored how to transfer learned knowledge across tasks or domains. Plenty of approaches have focused on situations where the distributions of the features and labels have changed, but the task is the same (e.g., classification across the same categories). \ZL{Do you want to add some citations here?}. Cross-task transfer learning strategies, on the other hand, have been widely adopted especially in the computer vision community where features learned by a deep neural network on a large classification task have been applied to a wide variety of other tasks \cite{Donahue14icml}. 
    
Most of the prior cross-task transfer learning works, however, require labeled target data to learn classifiers for the new task. If labels of the target data are absent, there is little choice other than to apply unsupervised approaches such as clustering on the target data with pre-trained feature representations. In this paper, we focus on the question of what can be transferred (besides features) to support both cross-domain and cross-task transfer learning. We specifically show that the most basic component of clustering, a learned similarity function, can be successfully used to achieve both cross-task and cross-domain transfer. However, a robust algorithm for clustering data with noisy pairwise similarity is essential to reconstruct the target data clusters, and this is the key to our work. We present a novel end-to-end deep neural network for this purpose, along with an appropriate loss function. Our approach can jointly optimize the features and clustering, hence taking advantage of such side information in a robust way. Using this method, we show that unsupervised learning can benefit from learning performed on a distinct task, and present an approach that transfers this side information from a labeled auxiliary data to an unlabeled domain in a different task. 

By formulating our approach as a deep neural network, one can easily add a classification loss into the framework. The setting then become similar to domain adaptation which transfers classifiers from a labeled source domain to an unlabeled target domain of the same task (which is available during training). In this configuration, each cluster output by our clustering network will be explicitly assigned to a category defined in the source domain during training. The major difference to previous domain adaptation work is that we transfer more information from the auxiliary data by learning a pairwise similarity prediction function, and we do not explicitly align source and target distributions. 

We demonstrate experimental results for both the unsupervised cross-transfer and domain adaptation tasks. For cross-task learning, we use the Omniglot dataset to show that we can achieve state of art clustering results when combining our transferred similarity prediction network and clustering loss using pair-wise constraints. For domain adaptation, we demonstrate improvements over state of art even when not performing any explicit domain adaptation (i.e. we do not have the unlabeled target data during training). We further show improved results when combining our idea with explicit domain adaptation, i.e. when the classification loss on the target labels is combined with joint optimization of the constrained clustering loss as well as a distribution similarity loss. Finally, we show that even when not transferring features themselves (i.e. pre-training the networks using ImageNet), we can achieve state of art cross-domain transfer for the SVHN-to-MNIST transfer task.



==> sections/method.tex <==
\section{What to Transfer?}
\subsection{Semantic similarity function}
In the cross-task problem, the object categories differ between source and target and hence there is a question of what to transfer from the source domain. While traditionally features can be transferred, this information is difficult to use in a manner that actually leverages the unlabeled information in the target domain. For example, performing unsupervised clustering on the features extracted from the unlabeled data only learns the best assignment of clusters given a fixed feature space and distance metric. In this paper, in addition to transferring features we transfer {\it semantic similarity} as a function $S(x_i,x_j)$, which takes a pair of data $x_i$ and $x_j$, and outputs a binary prediction $p\in\{similar,dissimilar\}$. The key insight is that, given an appropriate clustering algorithm that can jointly optimize features and cluster assignments given weak pair-wise constraints, the knowledge encoded in $S$ can be used not just to cluster but also to {\it optimize the features} for clustering. Note that this is similar to distance metric learning, except that we jointly optimize with cluster assignments as well.

\YH{Candidate to remove We hypothesize that one can learn a generalizable function to distinguish whether a pair of data belong to the same semantic category, assuming there is a sufficient number of classes to learn such a function. With the requirement that a large number of categories should be available during training, our similarities are learned from Omniglot[ref] and ImageNet[ref], which has 1623 alphabets and 1000 object categories respectively. Details are described in later sections.}

\subsection{Pairwise Similarity Prediction Network} \label{PSPN}
Although there is no restriction of how $S(x_i,x_j)$ should be constructed, we choose deep convolution neural networks due to their efficiency in vision tasks. We design a network architecture inspired from \cite{zagoruyko2015learning}. While they use it to predict the image patch similarity, we use it to predict image-level semantic similarity. A major difference is that the Siamese architecture used in \cite{zagoruyko2015learning} is not efficient in both training and inference, especially when dense pairwise information is used. Therefore, instead of using Siamese architecture, we keep the single column backbone but add a pair-enumeration layer on top of the feature extraction network. The pair-enumeration layer will enumerate all pairs of feature vectors within a mini-batch and concatenate features. Suppose the input of the layer is $10*512$ while the mini-batch size is $10$ and the feature dimension is $512$, the output of the pair-enumeration layer will be $100*1024$. The back-propagation of the layer is also implemented to make sure gradients will flow through the corresponding input features.

The full architecture is illustrated in Figure [X]. One hidden fully connected layer was added on top of the enumeration layer and a binary classifier was also added at the end. We use the standard cross-entropy loss and train it end-to-end. The supervision for training was obtained from converting the ground-truth category labels, i.e, if two samples are from the same class then their label will be $similar$, otherwise $dissimilar$. The inference is also end-to-end and  outputs predictions among all pairs in a mini-batch. The output probability is between zero and one where one means more similar. We simply binarize at $0.5$ to obtain discrete predictions. In the following sections we simplified the notation of the pairwise similarity prediction network as $S$. Once $S$ is learned, it is then used as a static function in our experiments.

\section{How to Transfer?}
Compared to the straightforward method of transferring feature representations, utilizing pairwise information is non-trivial. Here we propose to use it as a weak or noisy supervision for target data. Note that in this work, we assume there is no label available for the target. Therefore the weak supervision is only obtained via feeding target data into $S$, which is learned using only source data. Since utilizing $S$ requires it to be able to make reasonable predictions about semantic similarity, the source tasks have to be related to the target tasks. For example, they are both classification tasks on images or documents, but they do not necessarily have to contain the same set of categories. There is also no assumption about the distribution of the source or target datasets. In other words, domain shift is possible.

The above arguments support two different scenarios for knowledge transfer. The first is unsupervised cross-task transferring. We consider a simple but challenging case where the categories in the source data and target data are exclusive, which means no category in the target task is present in the source task. Further, there is no label available for the target data, so it is unsupervised. The second scenario is cross-domain transfer, Which is the same setting as unsupervised domain adaptation [ref] and the source and target datasets have the same categories but with different data distributions.

In the following sections we will present strategies to transfer pairwise semantic similarity across tasks and domains. Although there are differences in the two scenarios, we propose to use a common loss function to transfer pairwise knowledge. Inspired by constrained clustering, we formulate our loss function in a manner such that it can be used as a constrained clustering loss when used standalone. However, it can also be used as an additional term to be combined with other losses, for example cross entropy. Furthermore, the proposed loss could be easily added at the end of any networks used for classification; therefore it is highly flexible and can be combined with other approaches for transfer learning as we show in the experiments.
 
\subsection{The constrained clustering loss function (CCL)} \label{CCNloss}
Although many constrained clustering algorithms been developed, few of them are scalable with respect to the number of pairwise relationships. Further, none of them can be easily integrated into deep neural networks. Inspired by the work of \cite{Hsu16iclrw}, we construct a contrastive loss for clustering on the probability outputs of a softmax classifier. However, each output node does not have to map to a fixed category but instead each output node represents a probabilistic assignment of a data point to a cluster. The assignment between output nodes and clusters are formed stochastically during the optimization, and is  guided by the pairwise similarity. If there is a similar pair, their output distribution should be similar, and vice-versa.

Specifically, we use the pair-wise KL-divergence to evaluate the distance between cluster assignment distributions of two given input data, and use {\it predicted similarity} to construct the contrastive loss. Given a pair of data $\image{p}, \image{q}$, their corresponding output distributions are defined as $\mathcal{P}=\neuralnetwork{\image{p}}$ and $\mathcal{Q}=\neuralnetwork{\image{q}}$, while $f$ is the neural network. The cost of a similar pair is described as the KL-divergence between the distributions:
\begin{align}
\loss{\image{p}, \image{q}}^{+} &= \KL{\mathcal{P}^{\star} || \mathcal{Q}} + \KL{\mathcal{Q}^{\star} || \mathcal{P}} \\
\KL{\mathcal{P}^{\star}||\mathcal{Q}} &= \sum_{\clusters} {p_c log(\frac{p_c}{q_c})}
\end{align}
The cost $\loss{\image{p}, \image{q}}^{+}$ is symmetric w.r.t. $\image{p}, \image{q}$, in which $\mathcal{P}^{\star}$ and $\mathcal{Q}^{\star}$ are alternatively assumed to be constant.  Each KL-divergence factor $\KL{\mathcal{P}^{\star} || \mathcal{Q}}$ becomes a unary function whose gradient is simply $\partial \KL{\mathcal{P}^{\star} || \mathcal{Q}} / \partial \mathcal{Q}$. 

If $\image{p}, \image{q}$ comes from a pair which is defined as $dissimilar$, their output distributions are expected to be different, which can be defined as a hinge-loss function: 
\begin{align}
\loss{\image{p}, \image{q}}^{-} &= \hingeloss{\KL{\mathcal{P}^{\star}||\mathcal{Q}}, \sigma}  + \hingeloss{\KL{\mathcal{Q}^{\star}||\mathcal{P}}, \sigma} \\
\hingeloss{e, \sigma} &= max(0, \sigma - e)
\end{align}
Given a pair of data with similarity prediction $S(\image{p}, \image{q})\in\{similar, dissimilar\}$, the total loss can be defined as a contrastive loss as:
\begin{align}
\loss{\image{p}, \image{q}} = [S(\image{p}, \image{q})=similar] \loss{\image{p}, \image{q}}^{+} + [S(\image{p}, \image{q})=dissimilar]\loss{\image{p}, \image{q}}^{-} 
\end{align}
in which $[\cdot]$ is an Iverson Bracket. Given $S$ in the loss function, the contrastive loss can be end-to-end optimized together with the neural network. 

Since we can obtain dense pairwise information from $S$, to efficiently utilize the pair-wise information without forwarding each data multiple times we again using the pair-enumeration layer described in section \ref{PSPN}. Let $T$ be the set of all tuples $(i,j)$, while $i$ and $j$ are the indices of a sample in a mini-batch. The clustering loss $L_{clust}$ for a mini-batch is calculated by:
\begin{equation}
L_{clust} = \sum_{\forall{(i,j)}\in{T}}\loss{\image{i}, \image{j}}.
\end{equation}

\subsection{Transfer across tasks} \label{crosstask}
If the target task has different categories, we cannot directly transfer the classifier from source to target. Here we propose to first reduce the categorization problem to a surrogate same-task problem. We can directly apply transductive transfer learning \citep{Pan10pami} to the transformed task. The cluster structure in the target data are then reconstructed using the predictions in the transformed task.

The concept is illustrated in figure \ref{fig:crosstask}. The source involves a labeled auxiliary dataset $A=(X_A,Y_A)$, where $X_A$ is the set of data instances and $Y_A$ is the corresponding categorical labels. Further, we have an unlabeled target dataset $T=(X_T,Y_T)$, where $Y_T$ is the target that must be inferred. It is called cross-task if the set of categories $\{Y_A\}\neq\{Y_T\}$, and it is unsupervised since $Y_T$ is unknown. We first transform the problem of categorization into a pairwise similarity prediction problem. In other words, we specify a transformation function $R$ such that $R(A)=(X^R_A,Y^R)$, and $X^R_A=\{(x_{A,i},x_{A,j})\}_{\forall{i,j}}$ contains all pairs of data, where $Y^R=\{similar,dissimilar\}$. The transformation on the labeled auxiliary data is straightforward. It will be $similar$ if two data instances are from the same category, and vice versa. We then use it to learn a pairwise similarity prediction function $y_{i,j}=S(x_i,x_j)$. By applying $S$ on the $T$, we can obtain $S(x_{T,i},x_{T,j})=y_{T,i,j}$. The last step is to infer $Y_T$ from $Y^R_T=\{y_{T,i,j}\}_{\forall{i,j}}$, which can be solved by using constrained clustering algorithms. Note that since the actual $Y_T$ is unknown, the algorithm only infers the indices of categories, which could be in arbitrary order. The resulting clusters are expected to contain coherent semantic meanings.

\ZK{Candidate for removal: In general, discovering semantically-meaningful clusters from an unlabeled set of images is a hard problem. First, the feature space might not contain the information for distinguishing the human-defined categories. Second, the chosen distance metric might not reasonably estimate the semantic similarity. For example, using k-means to cluster images based on their raw pixels might produces clusters that are coherent in color instead of semantic category. In contrast, our framework uses learned constraints to guide the clustering. Therefore the images are aggregated and separated based on how we learn the similarity function $S$. In other words, the transferability is totally controlled by $S$. The better the generalization of $S$, the wider the range of tasks that our framework can be applied to.}

\subsection{Transfer across domains} \label{crossdomain}
The major difference in the cross-domain (same-task) setup is that the source data contains the same categories as the target data but with a potential domain shift. Thus the learned classifier can be transferred to the target directly. The problem setting we considered here is the same as unsupervised domain adaptation. Following the standard evaluation procedure \citep{LongZ0J17,ganin2016domain}, there are two labeled datasets in the source domain. The first one is usually just called source data which has the same set of labels as target. The second one is called the axillary data, which may or may not contains target categories, but has a large number of classes (e.g. ImageNet). The network is pre-trained with the axillary data, then fine-tuned with source data to learn the classifiers. To enhance the performance of the classifier on target data, some strategies can be applied to minimize the domain discrepancy between the training source and target data. Although aligning the distribution between two datasets is an effective approach, our experiment (in supplementary data) shows that simply using deeper pre-trained networks produces a significant performance boost by itself. Specifically, using Resnet-50 increases the performance 8.4 points from Alexnet, which surpasses the 6.2 points gained by using one of the state-of-the-art domain adaptation algorithms (JAN \citep{LongZ0J17}). If we regard pre-training with deeper networks as transferring more information, our approach is similar to this aspect since both transfer more information from the auxiliary dataset.

In this work we transfer the semantic similarity as the extra information from the auxiliary data. The scheme is illustrated in figure [X]. We simultaneously use CCL for target data while using classification loss for source data. The overall training procedure is similar to previous domain adaptation approaches in that both source and target data are mixed in a mini-batch, but different losses are applied. We denote the source domain images in a mini-batch $b$ as $X_{S,b}$ and the target domain images $X_{T,b}$ with its set of pairs $T_{T,b}$. The loss function $L_{da}$ for a mini-batch can then be formulated as:
\begin{equation}
	L_{da} = L_{cls} + L_{clust} \label{eq:Lda}
\end{equation}
While
\begin{equation}
	L_{cls} = \frac{1}{|b|}\sum_{\forall{\image{i}}\in{X_{S,b}}}{CrossEntropyLoss(f(\image{i}))}.
\end{equation}
and
\begin{equation}
	L_{clust} = \frac{1}{|b|^2}\sum_{\forall{(i,j)}\in{T_{T,b}}}\loss{\image{i}, \image{j}}.
\end{equation}
The $L_{clust}$ and $L_{cls}$ share the same outputs from network $f$. Although $L_{clust}$ does not force the mapping between clusters and categories, $L_{cls}$ does it. Therefore the learned classifier can be applied on target data directly and picks the maximum probability for the predicted class. Note that in our loss function, there is no term to explicitly match the feature distribution between source and target; it merely transfer more knowledge as constraints to regularize the learning of the classifier. There is also no requirement for the architecture to utilize hidden layers. Therefore our approach has large flexibility to be combined with other domain adaptation strategies, which we will demonstrate in the experiments.



==> sections/relatedwork.tex <==
\section{Related Work}

\cite{Pan10pami} introduces a comprehensive overview of transfer learning and extensively discusses "(1) What to transfer; (2) How to transfer; (3) When to transfer". Regarding "How to transfer", our work will focus on problems whose source domain and target domain are related but not the same. As for "What to transfer", we propose to transfer both features and a similarity metric that can be learned from any source task with strong or weak supervision and applied to a completely unsupervised task. In the following, we will discuss related work relating to "How to transfer".
% why we need transfer learning: transfer knowledge across different domain; data is out-dated. 

\paragraph{Cross-task Transfer Learning}  Learning from related tasks has been studied extensively as \emph{multi-task learning} \cite{Argyriou07nips}\cite{Caruana97ml}\cite{Jalali10nips}, \emph{learning to learn} or \emph{meta-learning} \cite{Andrychowicz16nips}\cite{Thrun98book}. \cite{Caruana97ml} presents the purpose of multi-task learning as improvement of generalization by incorporating domain-specific information shared across different tasks. \cite{Argyriou07nips} propose to optimize representations which can be efficiently shared by related tasks. With the success of deep learning, transferring pre-trained features to the target task is a widely used general approach, e.g. \cite{Donahue14icml, Yosinski14nips} The use of convolutional neural networks as representation learning has been a mainstay in many computer vision tasks \cite{Anastasia15cvpr}\cite{Yim15cvpr}\cite{Zhou17cvpr} etc. However the idea behind using multi-task learning to uncover the common latent features beneficial to each individual task is not our ultimately goal in transfer learning. Multi-task learning typically train on the source and target domains simultaneously with equal interests while the mission of transfer learning in general focuses more about the target task. In our work, we focus on transferring a weak form of information through a different task, with or without transferring features or adaptation. 

%\ZK{REMOVED as I'm not sure what this means:, and one usually has the labels for the task of interest}

% shows the application of transfer learning in different tasks
%Different layers in the learned deep models were shown to be general and benefit new tasks \cite{Oquab14cvpr}\cite{Razavian14cvprw}. 

\paragraph{Semi-supervised / Unsupervised Transfer Learning} There is a long tradition of learning algorithms that attempt to discover good feature representations for the task of interest using extra data from source or target domains \cite{Ando05jmlr}\cite{Mesnil12jmlr}. The work of transfer learning using unlabeled data is a popular setup \cite{Bengio11icutlw}\cite{Raina07icml}, which has also been called \emph{Self-taught learning}. Within this class of methods, extensive unsupervised learning work in the computer vision domain has been done, for example through auto-encoders \cite{Bengio09ftml}\cite{Hinton06science}, variational auto-encoders \cite{Kingma14iclr}, and generative adversarial networks \cite{Goodfellow14nips}. Many of these methods support both unsupervised and semi-supervised learning \cite{Arjovsky17arXiv}\cite{Kingma14nips}\cite{Mirza14arXiv}\cite{Radford15arXiv}. There is also work focusing on exploiting self-supervision as a self-teaching signal, such as context prediction \cite{Doersch15iccv}, image inpainting \cite{Pathak16cvpr}, motion from video \cite{Pathak17cvpr}, etc. However, there is a smaller body of work in transfer learning studying the use of a limited amount of labeled data to assist unsupervised learning. 

\paragraph{Constrained Clustering} A large body of work on purely unsupervised learning focuses on methods such as clustering. When certain prior knowledge is available as auxiliary information, constraint-based (or semi-supervised) clustering methods employ the existing labeled data to assist unsupervised learning \cite{Antoine12csda}. Previous work utilizing supervised data can be categorized majorly in two directions: 1) Using constraint-based methods to guide the clustering algorithms towards a better data grouping \cite{Wang14dmkd}\cite{Rangapuram15arXiv}\cite{Antoine14sc} and 2) learning an adapted similarity metric used by clustering algorithms \cite{Anand14pami} \cite{Davis07icml}. In constraint-based approaches, the clustering algorithm itself is modified so that  constraints are used to guide the algorithm towards a more appropriate data partitioning. This is done by modifying the clustering objective function so that it includes satisfaction of constraints. In metric-based approaches, an existing clustering algorithm that uses a distance metric is employed; however, the metric is first trained to satisfy the labels or constraints in the supervised data. \cite{Bilenko04icml} introduces K-means based algorithm incorporating both metric learning and the use of pairwise constraints in clustering approaches, which achieves a better result than a single type of supervision. 

Although there is extensive previous work studying the use of constrained clustering algorithms,  most of these works are semi-supervised approaches which uses a mixed of labeled data and unlabeled data in the same domain. Our motivation is conceptually different in that we achieve unsupervised clustering in the target domain by introducing constraints from a different domain, which are noisy. Further, our method jointly optimizes both the feature space and similarity metric (and hence clustering) using pair-wise constraints, and we achieve state of art clustering on unlabeled target domains when compared to the above clustering approaches.

